Patterns in the Chaos - a Study of Performance Variation and Predictability in Public IaaS Clouds

Benchmarking the performance of public cloud providers is a common research topic. Previous research has already extensively evaluated the performance of different cloud platforms for different use cases, and under different constraints and experiment setups. In this paper, we present a principled, large-scale literature review to collect and codify existing research regarding the predictability of performance in public Infrastructure-as-a-Service (IaaS) clouds. We formulate 15 hypotheses relating to the nature of performance variations in IaaS systems, to the factors of influence of performance variations, and how to compare different instance types. In a second step, we conduct extensive real-life experimentation on Amazon EC2 and Google Compute Engine to empirically validate those hypotheses. At the time of our research, performance in EC2 was substantially less predictable than in GCE. Further, we show that hardware heterogeneity is in practice less prevalent than anticipated by earlier research, while multi-tenancy has a dramatic impact on performance and predictability.

==> src/survey.tex <==
\section{Research Method}
\label{sec:survey}

The goal of our research is to identify the fundamental rules, patterns and mechanisms underlying the performance variations of public cloud systems.
Concretely, we are interested in the following three research questions:

\newcounter{qcounter}
\begin{list}{\textbf{RQ \arabic{qcounter}:}~}{\usecounter{qcounter}}
	\item What are the most common research outcomes that previous publications on IaaS benchmarking have reported?
	\item Which of those results stood the test of time, and can still be validated using an independent experiment setup?
	\item What research gaps still exist in literature?
\end{list} 

For RQ 1, we were specifically interested in rules, patterns, and mechanisms  (e.g, that I/O throughput tends to be less predictable than CPU performance), and not so much in concrete numerical measurements. That is, we already assumed going into this research that a concrete performance measurement taken in e.g., 2010 would not be accurate anymore at the time of this writing. However, our theory was that the underlying mechanisms, especially those reported by multiple researchers, would remain valid. We valided this assumption as part of our work on RQ 2, using our own experiment set and based on real-life numerical data collected on two different providers. Finally, in RQ 3, we identified research gaps that are not extensively covered to date. To address those questions, we have conduced a multi-phase empirical study, consisting of a systematic literature review, hypothesis building, data collection, and statistical hypothesis testing. We provide a complete literature list, all raw data, benchmark code, and more detailed analysis on the companion website to this paper\footnote{\url{http://wp.ifi.uzh.ch/leitner/www14}}. 

\subsection{Systematic Literature Review}
At the beginning of our research, we used a systematic literature review (as known from Evidence-Based Software Engineering~\cite{kitchenham:04})
to collect the existing state of research on IaaS benchmarking. We seeded our literature review with 7 seminal publications, which we considered widely-known and representative of the field going into the study~\cite{phillips:11,schad:10,lenk:11,mao:12,iosup:11,imai:13,fittkau:12}. We also added two of our own earlier publications to the initial seed for our literature review~\cite{borhani:14,scheuner:14}. From those 9 primary studies, we then generated a candidate set of additional relevant studies by following all backward (\emph{Which other studies does this publication reference?}) and forward references (\emph{Which other studies are referencing this publication?}). We used the Google Scholar\footnote{\url{http://scholar.google.com}} online service to identify forward references, as our experience is that Google Scholar maintains a more extensive publication list than any of the digital libraries of scientific publishers. From the resulting (oftentimes quite large) set of additional candidate studies, we accepted those that were after initial screening of paper title and abstract (1) specifically about benchmarking \emph{public} cloud services (we disregarded studies on private cloud systems or self-hosted data centres, as studies and results are generally quite different if the researchers also have access to the physical machines hosting the benchmarked resources), and (2)  which additionally explicitly reported numerical performance data (we disregarded studies that report on having conducted benchmarking as part of their research, but do not explicitly report their results). We have repeated this process three times, until we were unable to find additional relevant studies using this methodology. This resulted in a collection of 56 studies relevant to public cloud benchmarking. A full list is available in our companion website.         

\begin{figure}[h!]
\centering
 \includegraphics[width=0.75\linewidth]{img/litsearch}
 \caption{Literature Search Procedure}
 \label{fig:search}
\end{figure}

We have used random sampling to validate the collected study set by verifying for 10 arbitrary relevant papers found by searching the ACM Digital Library\footnote{\url{http://dl.acm.org}} that they are indeed contained. 

% In \emph{Phase 1}, we used a structured literature search approach loosely based on the idea of systematic literature reviews known from Evidence-Based Software Engineering~\cite{kitchenham:04}. As a starting point, in \emph{Step 1.1}, we used the 46 relevant primary studies identified in~\cite{li:12}, and extended this initial collection of potentially relevant research with (a) a small number of works personally known to the authors (mostly, we seeded our paper collection with highly cited seminal works, such as~\cite{schad:10,iosup:11}), and (b) potentially relevant search results found by searching IEEEXplorer\footnote{\url{http://ieeexplore.ieee.org/Xplore/home.jsp}} and the ACM Digitial Library\footnote{\url{http://dl.acm.org}} using the keywords ``cloud service benchmarking'' and ``IaaS  benchmarking''. This generated a large set initial collection of research, which we, in \emph{Step 1.2}, further extended by iterating over all publications and following both forward and backward references,  adding all papers whose title and/or abstract seemed relevant. Forward references
% % (that is, later publications that have cited the publication in question)
% have been identified using Google Scholar\footnote{\url{http://scholar.google.com}}. We repeated this process until no new publications could be found. In \emph{Step 1.3} we then decided to aggressively filter this large collection of publications using the following conditions:
% 
% \begin{enumerate}
%   \item Include papers $iff$ they are explicitly and specifically about
% benchmarking public IaaS cloud services that deliver virtualized computing resources. Exclude work about benchmarking generic networked applications, in-house data centers, as well as work about benchmarking other types of cloud services.
% \item Include papers $iff$  the main contribution was about benchmarking. Concretely, we decided to exclude publications that consider benchmarking only as a precondition or sidenote (e.g.,~\cite{imai:13}), as those papers often leave out too much details about their benchmarking methodology to be of value to us. 
% \end{enumerate}
% 
% Clearly, for both rules, judgement calls had to be made. For instance, we have decided to include~\cite{roloff:12} despite being mainly about benchmarking the Windows Azure\footnote{\url{http://azure.microsoft.com/en-us/}} PaaS system, as the publication also contains valuable insights into EC2 and the IaaS backend used by Azure. This process delivered a much smaller set of 26 publications, which we considered the core \emph{Body of Research} for the remainder of the work. While not nearly as comprehensive as the original paper collection, this smaller Body of Research proved to be easier to handle and compare, and more directly relevant to our stated goals. We provide a complete list of these publications as part of an online appendix\footnote{\url{https://bitbucket.org/sealuzh/www14-online-appendix}}.
% 

Upon inspection of those 56 studies, it became evident that  there are clear trends underlying the results of different authors and research teams. Hence, we have used open coding to group and classify the core messages of different studies into codes, and formulated a set of 11 hypotheses. These hypotheses relate to the fundamentals of performance variability in public cloud systems, which factors influence the observed performance variability, and how instance types differ. We introduce the hypotheses we formed in Section~\ref{sec:observations}. 

% In \emph{Phase 2}, on initial inspection, it became evident that, despite differing numerical results, there are clear trends underlying the results of different authors and research teams. Hence, in \emph{Step 2.1}, we have screened the Body of Research, extracted what we considered the core messages and results of each paper, and aggregated them into 4 groups of high-level observations and hypotheses. In \emph{Step 2.2}, we refined these initial observations, and generated a set of \emph{13} working hypotheses and observations. We report on our findings in Section~\ref{sec:observations}.
% %We argue that these findings serve as a condensed version of the major results  achieved by existing research on public IaaS benchmarking.
% Note that these findings are not concerned with concrete ``numbers'' (i.e., what concrete benchmark results a paper has presented for a given cloud provider configuration), but with more general underlying concepts, such as variability of benchmark results, principles of cost effective cloud usage, and the idea of placement gaming. Further, not all reported hypotheses have been directly formulated in existing research. In some cases, we have come to new conclusions by observing the results presented in different papers, and speculating over the underlying commonalities and differences. 

\subsection{Data Collection}

We used Cloud Workbench~\cite{scheuner:14} to set up and collect a significant amount of performance measurements from
two real-life clouds (Amazon EC2 and Google Compute Engine). Based on our literature review,
we decided to execute 3 micro-benchmarks, targeting \emph{instance processor speed} (CPU), \emph{disk read/write speed} (IO), and
\emph{memory read/write speed} (MEM). Additionally, we defined two application benchmarks, measuring \emph{database queries per minute} (OLTP)
and \emph{the Git checkout and Java compilation time of an open source project} (Java). More details on these benchmarks is given in Table~\ref{tab:benchmarks}. All EC2 benchmarks used the official Ubuntu 14.04 LTS image from Canonical as base operating system. In GCE, currently no officially maintained Ubuntu images are available. Hence, we used Debian 7 Wheezy base images for this provider.

\begin{table}[h!]
\centering
\scriptsize
\begin{tabular}{|c|p{5.5cm}|c|}
	\hline
  \rowcolor[HTML]{EFEFEF} \textbf{Name} & \textbf{Description} & \textbf{Unit}\\
  \hline
  CPU & Uses \texttt{sysbench} to check 20000 natural numbers for prime-ness; measures time to completion & s \\
  \hline
  IO & Uses \texttt{sysbench} to repeatedly read / write a 5 GByte file for 3 minutes; measures average disk bandwith & Mb/s \\ 
  \hline
  MEM & Uses \texttt{mbw} to 50 times allocate two 64 MiB arrays in memory and copy one array to the other; measures average memory bandwidth &  MiB/s \\
  \hline
  OLTP & Uses \texttt{sysbench} to repeatedly execute SQL queries against a MySQL database with 10.000 rows for 3 minutes; measures average queries per second & queries/s \\   
    \hline
  Java & Clones a mid-sized Java project from GitHub and compiles it using OpenJDK 7; measures end-to-end duration & s \\   
  \hline
%   \hline
%   \texttt{io} & sysbench & micro &  Reads and writes large files from/to hard disk & \ldots bandwith when reading from and writing to hard disk & HIB & ? \\
%   \hline
% \texttt{oltp} & sysbench & application &  Executes SQL queries on a MySQL database & \ldots number of queries that can be executed in 10 minutes & HIB & Queries / Second \\
%   \hline
% \texttt{compile} & Git, Maven, OpenJDK 7 & application &  Clones a Java project from GitHub and builds it with Maven & \ldots duration of the checkout and build process & LIB & Seconds \\
\end{tabular}
\caption{Used Benchmarks}
\label{tab:benchmarks}
\end{table}

Further, we considered two types of experiments. In \emph{isolated tests}, we acquired a specific type of virtual resource from a provider, provisioned the benchmark code in this resource (e.g., installed the sysbench tool for the CPU benchmark), executed the benchmark three times directly after each other, and then immediately released the resource again. Using Cloud Workbench, we scheduled this procedure in various configurations on EC2 and GCE 6 times per day over a period of one month. Table~\ref{tab:data} lists the defined benchmarks and exact used configurations, as well as the exact number of collected measurements. Note that the numbers do not generally add up to the theoretical
number of 540 measurements, as we had to deal with regular transient faults, such as timeouts when interacting with the cloud provider. \textbf{TODO -- why do we actually have more data in some cases?}
In these cases, we have simply discarded the resulting measurements. 

\begin{table}[h!]
\centering
\scriptsize
\begin{tabular}{|l|l|l|l|l|l|l|l}
\hline
\rowcolor[HTML]{EFEFEF} & \textbf{Region} & \textbf{Type} & \textbf{CPU} & \textbf{IO} & \textbf{MEM} & \textbf{OLTP} & \textbf{Java} \\
\hline
\multirow{16}{*}{\rotatebox[origin=c]{90}{\textbf{EC2}}} & eu-west-1 & t1.micro & 501 & 613 & 615 & 498 & 618 \\
\cline{3-4}
 &  & m1.small & 489 & 595 & 588 & 486 & 582 \\
\cline{3-8}

\end{tabular}
\caption{Number of Collected Data Points per Configuration in \emph{Isolated Tests}}
\label{tab:data}
\end{table}	


\begin{table}[h!]
	\centering
	\scriptsize
	\begin{tabular}{|l|l|l|l|l|l|l|l|}
		\hline
		\rowcolor[HTML]{EFEFEF} & \textbf{Region} & \textbf{Type} & CPU & IO & MEM & OLTP & Java \\
		\hline
		\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{EC2}}} & eu-west-1 & t1.micro & 501 & 613 & 615 & 498 & 618 \\
		\cline{3-8}
		 & & m1.small & 489 & 595 & 588 & 486 & 582 \\
		\hline		
	\end{tabular}
	\caption{Number of Collected Data Points per Configuration in \emph{Isolated Tests}}
	\label{tab:data}
\end{table}		

Orthogonal to these isolated tests, we also collected data related to the performance stability of cloud resources
over time. For these \emph{continuous tests}, we again acquired a specific type of virtual resource
from a provider and provisioned the benchmark. However, we then continuously executed the benchmark every hour for a
total duration of 3 days (72 executions), after which we discarded the cloud resource again. For each benchmarked
configuration, we repeated this for 15 instances. The configurations used for these experiments are given in
Table~\ref{tab:data2}.

\begin{table}[h!]
\centering
\scriptsize
\begin{tabular}{|l|l|l|l|}
\hline
\rowcolor[HTML]{EFEFEF} & \textbf{Region} & \textbf{Type} & \textbf{Benchmarks(\# Data Points)} \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{EC2}}} & eu-west-1 & t1.micro & CPU(1080) IO(1080) MEM(1080) \\
\cline{3-4}
 &  & m1.small & CPU(1080) IO(1080) MEM(1080) \\
\cline{3-4}
 &  & m3.large & CPU(1080) IO(1080) MEM(1080) \\
\hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{GCE}}} & eu-west1-a & f1-micro & CPU(1080) IO(1080) MEM(1080) \\
 &  & n1-standard-1 & CPU(1080) IO(1080) MEM(1080) \\ 
 \cline{3-4}
 &  & n1-standard-2 & CPU(1080) IO(1080) MEM(1080) \\
  \hline
\end{tabular}
\caption{Number of Collected Data Points per Configuration in \emph{Continuous Tests}}
\label{tab:data2}
\end{table}	

The online companion of this paper contains all the benchmark code and Chef~\cite{chef} recipes to provision the
cloud instances in the exact configuration we used in our experiments. Further, we provide two data files containing
all raw data listed in Table~\ref{tab:data} and Table~\ref{tab:data2}. In Section~\ref{sec:experiments}, we use
this data to validate the hypotheses formed in Section~\ref{sec:observations}.

% % We introduce CWb in more detail in Section~\ref{sec:tool}.
% We defined benchmarks specifically with the idea of statistical validation of our formulated working hypotheses from Section \ref{sec:observations} in mind. Hence, in \emph{Step 3.2}, we did statistical analysis of our hypotheses. We detail our experiment setup as well as the results we achieved in Section~\ref{sec:experiments}, give a brief overview over related work in Section~\ref{sec:related}, and finally provide conclusions as well as threads to validity and limitations of our work in Section~\ref{sec:conclusions}.  

%\input{src/tables/benchmarks}		

% In order to collect enough base data to allow for statistically significant hypothesis testing, we selected an array of 5 micro- and application benchmarks, as summarized in Table~\ref{tab:benchmarks}. Three micro-benchmarks are used to gather data about the raw CPU, memory bandwidth, and hard disc read/write speed of cloud instances. Two example application benchmarks are used to get a more end-to-end view of the performance in different usage scenarios. Firstly, we use the \texttt{sysbench} utility to execute an ``OLTP'' test, which repeatedly executes SQL queries on a MySQL database management system. Secondly, we have self-defined a second application benchmark, which uses Git to clone a Java project from GitHub and compiles it using Maven. Note that for the \texttt{cpu} and \texttt{compile} benchmarks, a lower benchmark value is better, while a higher value is better for all other benchmarks.  
% 
% In order to test our hypotheses, we chose two popular public cloud providers, namely Amazon EC2 and Google Compute Engine (GCE). EC2 is a ``safe'' choice, as most existing research was also conducted on top of this provider. Further, we chose GCE due to being an (at the time of this writing) new high-profile player on the market, which is not covered at all by the current state of research. On both providers, we selected 3 common general-purpose instance types (\texttt{t1.micro} and \texttt{f1-micro}, \texttt{m1.small} and \texttt{n1-standard-1}, and \texttt{m3.large} and \texttt{n1-standard-2}), as well as two special types on EC2 (\texttt{c3.large} and \texttt{i2.xlarge}). For both providers, we ran our experiments on one data centre in the US (\texttt{us-east-1} and \texttt{us-central1-a}) as well as one in europe (\texttt{eu-west-1} and \texttt{europe-west1-a}). To reduce the costs of our experiments, we have not looked at special instance types in GCE, and used only the europe region in AWS. Further, we have executed the \texttt{oltp} and \texttt{mem} benchmarks only on AWS. 
% 
% We chose an Infrastructure-as-Code (IaC) approach to foster reproducability of our results. Each benchmark was defined as an Opscode Chef cookbook. Each cloud configuration was defined using Vagrant. Each experiment run then consisted of: (1) getting a fresh VM using the correct configuration from the provider using Vagrant, (2) automatically provisioning the right software (e.g., benchmarking code) using Chef, (3) running the benchmark three times, and submitting the results and some meta-information back to a central benchmarking tool, and (4) releasing the VM again. For each benchmark and configuration, we repeated this process 6 times a day for a duration of one month during July 2014. All in all, this delivered a data set of close to 30000 individual measurements, which we refer to as the \emph{basic} data in the following.
% 
% The \emph{basic} data set forms the basis of most of our analysis. However, for some hypotheses (e.g., \ref{hyp:perfvar_micro} or \ref{hyp:hardwarecorlongterm}), different data was needed. Hence, we have also collected two additional data sets. Firstly, we have collected an additional \emph{combined} data set (close to 7500 measurements), which has been collected similarly to the \emph{basic} data set, with the core difference that we used only the micro benchmarks, and that we deployed all benchmarks on the same virtual machine and executed them directly after each other. This data set was mostly to see whether there is a correlation between different micro benchmarks executed on the same virtual machine. Secondly, we have collected a \emph{longterm} data set. For this data, we have again only deployed micro benchmarks, this time on AWS only. The core difference in this data is that we have not terminated and re-acquired the used cloud virtual machines between runs. Instead, we kept virtual machines running and executed all micro benchmarks every hour for a total duration of 3 days. The main goal of this data was to be able to see whether the performance of virtual machines is stable over time. We have collected more than 3000 individual measurements this way.  All in all, this is the (to the best of our knowledge) most comprehensive IaaS performance study conducted in scientific literature so far. We provide all three data sets, as well as the Chef cookbooks, Vagrantfiles and tooling used to produce them, online for further academic analysis and validation of our results\footnote{TODO}.



==> src/tables/fig_cpu.tex <==
\begin{figure}[h]
\centering
 \includegraphics[width=\linewidth]{img/cpulong_fig5}
 \caption{\texttt{cpu} Benchmark Values over Time for 2 Example Executions}
 \label{fig:cpu_per_time}
 
% full.lineplot.cpu.single <- function(batch1, batch2) {
%   longterm_filtered <- subset(longterm, (longterm$Batch == batch1) | (longterm$Batch == batch2))
%   .e <- environment()
%   ggplot(aes(x=Count, y=CPUNormalValue, group=Batch, colour=factor(Batch)), data = longterm_filtered, environment = .e) + geom_line() + geom_point() +
%     ylab("(-1 * Time) [Seconds]") +
%     xlab("Experiment Runtime [Hours]") +
%     scale_color_discrete(name  ="",
%                          breaks=factor(c(12544, 12978)),
%                          labels=c("Instance 12544 (aws.eu.micro.cpu)   ", "Instance 12978 (aws.eu.small.cpu)  "))+
%     theme(legend.position="top", legend.text = element_text(size = 14), axis.text=element_text(size=15), axis.title=element_text(size=15,face="bold",vjust=0.1))
%   
% }
% full.lineplot.cpu.single(12544,12978)
 
\end{figure}

==> src/tables/fig_io.tex <==
\begin{figure}[h]
\centering
 \includegraphics[width=\linewidth]{img/iolong_fig4}
 \caption{\texttt{io} Benchmark Values over Time for 2 Example Executions}
 \label{fig:io_per_time}
 
%  full.lineplot.io.single <- function(batch1, batch2) {
%   longterm_filtered <- subset(longterm, (longterm$Batch == batch1) | (longterm$Batch == batch2))
%   .e <- environment()
%   ggplot(aes(x=Count, y=IOValue, group=Batch, colour=factor(Batch)), data = longterm_filtered, environment = .e) + geom_line() + geom_point() +
%     ylab("Bandwith [MBit / Second]") +
%     xlab("Experiment Runtime [Hours]") +
%     scale_color_discrete(name  ="",
%                          breaks=factor(c(9097, 14704)),
%                          labels=c("Instance 9097 (aws.eu.large.io)   ", "Instance 14704 (aws.eu.large.io)  "))+
%   theme(legend.position="top", legend.text = element_text(size = 14), axis.text=element_text(size=15), axis.title=element_text(size=15,face="bold",vjust=0.1))
%   
% }
%  full.lineplot.io.single(9097, 14704)
 
\end{figure}

==> src/tables/fig_variability.tex <==
\begin{figure*}[t!]
\centering
\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/cpu_fig1}
  \caption{CPU Benchmark Results}
  \label{fig:cpu}
\end{subfigure}

% included <- c("aws.eu.micro.cpu", "gce.eu.micro.cpu", "aws.eu.cpuopt.cpu", "aws.us.small.cpu", "gce.us.small.cpu")
% full.boxplot <- function(included) {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   isolated_filtered <- subset(isolated, isolated$Config %in% included)
%   .e <- environment()
%   g = ggplot(aes(y = isolated_filtered$NormalValue, x = isolated_filtered$Config), data = isolated_filtered, environment = .e) +
%     geom_boxplot() +
%     scale_y_continuous(limits = quantile(isolated_filtered$NormalValue, c(0.05, 0.95))) +
%     ylab("(-1 * Time) [Seconds]") +
%     xlab("Configuration [provider.region.size.benchmark]")
%   g+theme(axis.text=element_text(size=15), axis.title=element_text(size=15,face="bold",vjust=0.1))
% }
% full.boxplot(included)
% (export as PDF 3 inches high) 

\begin{subfigure}{\textwidth}
  \centering
  \includegraphics[width=\linewidth]{img/io_fig2}
  \caption{IO Benchmark Results}
  \label{fig:io}
\end{subfigure}

% included <- c("aws.eu.ioopt.io", "aws.us.large.io", "gce.us.large.io", "aws.us.small.io", "gce.us.small.io")
% full.boxplot <- function(included) {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   isolated_filtered <- subset(isolated, isolated$Config %in% included)
%   .e <- environment()
%   g = ggplot(aes(y = isolated_filtered$NormalValue, x = isolated_filtered$Config), data = isolated_filtered, environment = .e) +
%     geom_boxplot() +
%     scale_y_continuous(limits = quantile(isolated_filtered$NormalValue, c(0.05, 0.95))) +
%     ylab("Bandwith [MBit / Second]") +
%     xlab("Configuration [provider.region.size.benchmark]")
%   g+theme(axis.text=element_text(size=15), axis.title=element_text(size=15,face="bold",vjust=0.1))
% }
% full.boxplot(included)

\begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=\linewidth]{img/cpuhw_fig3}
    \caption{CPU Benchmarking Results per Served CPU Type}
    \label{fig:cpuhw}
\end{subfigure}

% included <- c("aws.eu.small.cpu", "aws.us.small.cpu")
% full.boxplot.cpu <- function(included) {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   isolated_filtered <- subset(isolated, isolated$Config %in% included)
%   .e <- environment()
%   g = ggplot(aes(y = isolated_filtered$NormalValue, x = gsub("Intel\\(R\\) Xeon\\(R\\) CPU ", "", isolated_filtered$CPU)), data = isolated_filtered, environment = .e) +
%     geom_boxplot() +
%     ylab("-(-1 * Time) [Seconds]") +
%     xlab("Self-Reported CPU Model")
%   g+theme(axis.text=element_text(size=15), axis.title=element_text(size=15,face="bold",vjust=0.1))
% }
% full.boxplot.cpu(included)

\caption{Basic Benchmark Results}
\label{fig:basic}
\end{figure*}	

==> src/tables/var_app.tex <==
\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{r|c|c|c|c|c}
 &  & \textbf{EC2/EU} & \textbf{EC2/US} & \textbf{GCE/EU} & \textbf{GCE/US} \\
  \hline
  \texttt{oltp} & micro & 0.31 & 0.32 & n/a & n/a \\
  & small & 0.13 & 0.16 & n/a & n/a \\
  & large &0.21 & 0.37 & n/a & n/a \\
  & cpu-opt &0.21 & n/a & n/a & n/a \\
  & io-opt &0.12 & n/a & n/a & n/a \\
\hline
\texttt{compile} & micro & 0.39 & 0.80 &0.37 &0.30 \\
  & small & 0.12 & 0.38 &0.10 & 0.14 \\
  & large & 0.15& 0.96 & 0.96 & 0.33 \\
  & cpu-opt &0.13 & n/a & n/a & n/a \\
  & io-opt &0.14 & n/a & n/a & n/a \\
    
  
%   full.rstd <- function() {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   configs <- unique(isolated$Config)
%   rstds <- c() 
%   for(c in configs) {
%     c_rstd <- rstd(c)
%     rstds[length(rstds)+1] <- c_rstd
%   }
%   data.frame(configs, rstds)
% }
% 
% rstd <- function(config) {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   filtered = subset(isolated, isolated$Config == config)
%   mean = mean(filtered$Value)
%   std = sd(filtered$Value)
%   return (std / mean)
% }
% 
% full.rstd()
  
\end{tabular}
\caption{Relative Standard Deviations of Application Benchmarks}
\label{tab:rstd_app}
\end{table}

==> src/tables/var_micro.tex <==
\begin{table}[t!]
\centering
\scriptsize
\begin{tabular}{r|c|c|c|c|c}
  & & \textbf{EC2/EU} & \textbf{EC2/US} & \textbf{GCE/EU} & \textbf{GCE/US} \\
  \hline
 \texttt{cpu} & micro & 0.12 &0.20  &0.05 &0.05 \\
  & small & 0.3 &0.12 &0.00 & 0.02\\
  & large & 0.00 &0.00 & 0.02& 0.01\\
  & cpu-opt & 0.00 & n/a & n/a & n/a\\
  & io-opt & 0.00 & n/a & n/a & n/a\\
  \hline   
\texttt{mem} & micro & 0.18 &0.26  & n/a & n/a \\
 & small & 0.04  & 0.26  & n/a & n/a \\
 & large & 0.02 & 0.04  & n/a & n/a \\
  & cpu-opt & 0.09 & n/a & n/a & n/a \\
  & io-opt & 0.12 & n/a & n/a & n/a \\  
  \hline
  \texttt{io} & micro & 7.70 &5.58 &0.03 & 0.09\\
  & small & 3.26& 0.94& 0.03& 5.81\\
  & large & 0.36& 2.01& 0.57& 0.53\\
  & cpu-opt & 0.59& n/a& n/a& n/a\\
  & io-opt & 0.20& n/a& n/a& n/a\\
    
  
%   full.rstd <- function() {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   configs <- unique(isolated$Config)
%   rstds <- c() 
%   for(c in configs) {
%     c_rstd <- rstd(c)
%     rstds[length(rstds)+1] <- c_rstd
%   }
%   data.frame(configs, rstds)
% }
% 
% rstd <- function(config) {
%   isolated$Config = interaction(isolated$Cloud, isolated$Region, isolated$Size, isolated$Benchmark)
%   filtered = subset(isolated, isolated$Config == config)
%   mean = mean(filtered$Value)
%   std = sd(filtered$Value)
%   return (std / mean)
% }
% 
% full.rstd()
  
\end{tabular}
\caption{Relative Standard Deviations of Micro-Benchmarks}
\label{tab:rstd_micro}
\end{table}

==> src/test.tex <==








\textbf{Formalization}\\
\\
\textbf{Isolated}
\begin{equation}
\begin{split}
c \in \mathcal{C}\\
c = \langle \mathcal{P}, \mathcal{R}, \mathcal{T}, \mathcal{B} \rangle\\
\mathcal{P} = \{ aws, gce \}\\
\mathcal{R} = \{ us, eu \}\\
\mathcal{T} = \{ micro, small, large, cpuopt, ioopt \}\\
\mathcal{B} = \{ \text{CPU, MEM, Java, IO, OLTP} \}\\
\\
i\colon \mathcal{C} \mapsto \mathcal{I}\\
i(c) \in \mathcal{I}\\
\\
m\colon \mathcal{I} \mapsto \mathbb{R}
m(i) \in \mathbb{R}\\
m_{c,ht}(i) \subseteq m(i)
\\
m_{c,E5655}
\end{split}
\end{equation}
\\
\textbf{Longterm}
\begin{equation}
\begin{split}
c_l \in \mathcal{C}_l\\
c_l = \langle \mathcal{P}, \mathcal{R}, \mathcal{T}_l, \mathcal{B}_l \rangle\\
\mathcal{T}_l = \{ micro, small, large \}\\
\mathcal{B}_l = \{ CPU, MEM, IO \}\\
\\
i_l(c_l) \in \mathcal{I}\\
m_l(i_l) \in \mathbb{R}
\end{split}
\end{equation}

==> src/tool.tex <==
\section{Experimental Setup}
\label{sec:tool}

\subsection{Cloud Benchmark Toolsuite}
TODO

Proin mattis justo nec posuere viverra. Quisque scelerisque augue tempor, consequat eros eu, condimentum libero. Phasellus tempus neque vel ante placerat, et scelerisque elit elementum. Aliquam erat volutpat. Proin vel nisi rutrum, suscipit odio vitae, porta dolor. Integer tincidunt tortor vitae dictum congue. Maecenas tincidunt elementum porttitor. Phasellus pretium feugiat metus ac lobortis. Pellentesque eleifend egestas sem, nec commodo justo pellentesque id. In ac tortor eu sapien laoreet pulvinar.

Quisque id sodales mauris. Nulla facilisi. Maecenas sit amet auctor tellus, ut cursus augue. Donec eu neque sed nisi commodo ultricies in at enim. Aenean volutpat iaculis commodo. Integer facilisis lacus nec lectus rutrum interdum in a nisl. Curabitur quis sem non est tristique porttitor sed mattis nulla.

Quisque sagittis ipsum vitae ultricies gravida. Curabitur ac sem eu purus interdum tincidunt. Cum sociis natoque penatibus et magnis dis parturient montes, nascetur ridiculus mus. Morbi risus ligula, dapibus ac venenatis vitae, tincidunt quis dui. Suspendisse mi leo, volutpat vel bibendum non, tincidunt vitae odio. Duis aliquet quis mauris id sodales. Maecenas suscipit accumsan augue a feugiat. Nulla eget mollis justo, eget dignissim massa. Nunc in viverra purus, sit amet pharetra urna. Phasellus molestie nulla sed feugiat dictum. Duis fringilla tellus eu nunc porttitor volutpat. Suspendisse nec ligula id nulla luctus convallis nec ut odio. Mauris eget tristique nisl. Proin ultrices, nisl vulputate porta lobortis, libero ante aliquam lorem, et adipiscing risus massa et nibh. In eget imperdiet ipsum. Nunc egestas eu neque id aliquam.
